VLABench: A Large-Scale Benchmark for Language-Conditioned Robotics Manipulation with Long-Horizon Reasoning Tasks

General-purposed embodied agents are designed to understand the users' natural instructions or intentions and act precisely to complete universal tasks. Recently, methods based on foundation models especially Vision-Language-Action models (VLAs) have shown a substantial potential to solve language-conditioned manipulation (LCM) tasks well. However, existing benchmarks do not adequately meet the needs of VLAs and relative algorithms. To better define such general-purpose tasks in the context of LLMs and advance the research in VLAs, we present VLABench, an open-source benchmark for evaluating universal LCM task learning. VLABench provides 100 carefully designed categories of tasks, with strong randomization in each category of task and a total of 2000+ objects. VLABench stands out from previous benchmarks in four key aspects: 1) tasks requiring world knowledge and common sense transfer, 2) natural language instructions with implicit human intentions rather than templates, 3) long-horizon tasks demanding multi-step reasoning, and 4) evaluation of both action policies and language model capabilities. The benchmark assesses multiple competencies including understanding of mesh\&texture, spatial relationship, semantic instruction, physical laws, knowledge transfer and reasoning, etc. To support the downstream finetuning, we provide high-quality training data collected via an automated framework incorporating heuristic skills and prior information. The experimental results indicate that both the current state-of-the-art pretrained VLAs and the workflow based on VLMs face challenges in our tasks.

==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> table/asset.tex <==
\renewcommand{\arraystretch}{1.2}
% TODO
\begin{table}[t]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
    Name & Category Number & Asset Number \\ \hline
    Billiards & 2 & 24 \\ \hline
    Billiards Table & 1 & 1 \\ \hline
    Books & 8 & 52 \\ \hline
    Baked Goods & 5 & 60 \\ \hline
    Coffee Machine & 1 & 5 \\ \hline
    Condiment & 5 & 50 \\ \hline
    Box Container & 1 & 10 \\ \hline
    Cabinet & 1 & 5 \\ \hline
    Cutting Board & 1 & 15 \\ \hline
    Fridge & 1 & 5 \\ \hline
    Microwave & 1 & 5 \\ \hline
    Safe & 1 & 5 \\ \hline
    Shelf & 1 & 10 \\ \hline
    Stove & 1 & 5 \\ \hline
    Tray & 1 & 15 \\ \hline
    Vase & 1 & 10 \\ \hline
    Counter & 1 & 20 \\ \hline
    Dessert & 4 & 58 \\ \hline
    Drink & 9 & 130 \\ \hline
    Flower & 9 & 25 \\ \hline
    Fruit & 11 & 227 \\ \hline
    Ingredient & 16 & 181 \\ \hline
    Mahjong & 1 & 38 \\ \hline
    Number Cube & 1 & 10 \\ \hline
    Painting & 1 & 286 \\ \hline
    Poker & 1 & 54 \\ \hline
    Snack & 8 & 97 \\ \hline
    Table & 1 & 20 \\ \hline
    Tableware & 11 & 216 \\ \hline
    Tool & 9 & 49 \\ \hline
    Toy & 35 & 140 \\ \hline
    Chemistry Solution & 1 & 30 \\ \hline
    Name Tag & 1 & 30 \\ \hline
    Flask & 1 & 5 \\ \hline
    Tube Container & 1 & 1 \\ \hline    
    \textbf{Total} & 163 & 2164 \\ \hline
    
    
    \end{tabular}
    \caption{\textbf{Assets statics}. Statistics of object categories and the number of objects used in VLABench. }
    \label{tab:asset}
\end{table}

==> table/asset_two_column.tex <==
\begin{table}[t!]
    \centering
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{|c|c|c||c|c|c|}
    \hline
    Grasp Obj & N-Cate & N-Obj & Recep & N-Cate & N-Obj\\ \hline
    Billiards & 2 & 24 & Billiards Table & 1 & 1 \\ \hline
    Books & 8 & 52 & Shelf & 1 & 10 \\ \hline
    Baked Goods & 5 & 60 & Microwave & 1 & 5 \\ \hline    
    Condiment & 5 & 50 & Cabinet & 1 & 5 \\ \hline
    Dessert & 4 & 58 & Tray & 1 & 15 \\ \hline
    Drink & 9 & 130 & Fridge & 1 & 5 \\ \hline
    Flower & 9 & 25 & Vase & 1 & 10 \\ \hline
    Fruit & 11 & 227 & Box Container & 2 & 10 \\ \hline
    Ingredient & 16 & 181 & Cutting Board & 1 & 15 \\ \hline
    Mahjong & 1 & 38 & Counter & 1 & 20 \\ \hline
    Number Cube & 1 & 10 & Safe & 1 & 5\\ \hline
    Painting & 1 & 286 & Stove & 1 & 5 \\ \hline
    Poker & 1 & 54 & Table & 1 & 20 \\ \hline 
    Snack & 8 & 97 & Juicer & 1 & 3\\ \hline
    Flatware & 4 & 80 & Crockery & 7 & 136\\ \hline
    Tool & 9 & 49 & Coffee Machine & 1 & 5\\ \hline
    Toy & 35 & 140 & Placemat & 1 & 10\\ \hline
    Chemistry Solution & 1 & 30 & Tube Container & 1 & 1\\ \hline
    Name Tag & 1 & 30 & Flask & 1 & 5 \\ \hline
    \end{tabular}}
    \caption{\textbf{Assets statics}. Statistics of object categories and the number of objects used in VLABench. }
    \label{tab:asset}
\end{table}

==> table/prompt.tex <==
% \onecolumn
% \begin{longtable}{p{2cm} p{3cm} p{12cm}}
%     \hline
%     \textbf{Task} & \textbf{Type} & \textbf{Prompt} \\ 
%     \hline
%     % Common Sense & World Knowlegde
%     1. Select Fruit & Common Sense & I am going to make some task instructions for a robot arm. Here are some target objects:xxx. And the target entity is xxx. The target entity is the object that the robotic arm is supposed to grasp, move, or perform other operations on. Our task requirements are related to the characteristics of the target object and should also reflect everyday needs for a specific item.
%     Please find the target entity's specific character which is different with other target objects and combine into the instruction.
%     For example: 'target\_entity: orange, instruction: I want a fruit that is the richest in vitamin C.'
%     Please provide the task following the format of the above example.
%     Please provide ten tasks that meet the above requirements and format.\\

%     2. Select Drink & Common Sense & I am going to make some task instructions for a robot arm. Here are some target objects (they are all drinks' names): xxx. And the target entity is xxx. The target entity is the one that the robotic arm is supposed to grasp, move, or perform other operations on. Our task requirements are related to the characteristics of the target object and should also reflect everyday needs for a specific item.
%     Please find target entity's specific character which is different with other target objects and combine into the instruction.
%     For example:
%     'target\_object: milk, instruction: I want a smooth beverage rich in calcium.'
%     Please provide the task following the format of the above example.
%     The target\_object must be the target entity. Please provide ten tasks that meet the above requirements and format.

%     3. Select Toy & Common Sense & I am going to make some task instructions for a robot arm. Here are some target objects (they are all toy names): xxx. And the target entity is xxx. The target entity is the one that the robotic arm is supposed to grasp, move, or perform other operations on. Our task requirements are related to the characteristics of the target object. The instruction should focus on IP, rather than directly saying which toy to choose.  
%     Please create tasks based on the specific characteristics of the recipient, combining them with the unique features and IP of the toys. Do not directly mention the target toy by name.
%     Please find target entity's specific character which is different with other target objects and combine into the instruction.   
%     For example: 'target_object: donald, instruction: 'I want a toy in the Disney series.''
%     'target\_object: goku, instruction: 'Pick a toy which is belong to the dragon ball.'' 
%     'target\_object: ironman, instruction: 'Select a toy in the Marvel series.''   
%     Please provide the task following the format of the above example.
%     The target_object must be the target entity. Please provide ten tasks that meet the above requirements and format.
    
%     % Semantically rich instruction
%     1. Select Fruit with User Requirement & Semantic Instruction & -- & -- & & The user expresses a need for a certain type of fruit during a semantically rich conversation, such as when making a strawberry cake. \\



%     % Physics laws
%     1. Friction QA & Physical Law & -- & -- &s & Choose the object with proper friction force based on the geometry shapes and materials. \\


    
%     % Complex tasks
%     1. Make Juice & Composite & The agent is required to understand the user's intention during a conversation and use a juicer to make proper juice. \\
    

    
%     \caption{Task List. Include the name, type, ability required, and detailed description of all the tasks.}
%     \label{table:task_description}
% \end{longtable}
% \onecolumn
\begin{tcolorbox}[colback=green!10, colframe=green!80!black, title=System Prompt]
I am going to make some task instructions for a robot arm. Here are some objects (they are all xxx' names):xxx. And the target entity is xxx. \textbf{\{Here, the xxx represents the object name for different tasks.\}}\\
The target entity is the object that the robotic arm is supposed to grasp, move, or perform other operations on. Our task requirements are related to the characteristics of the target object and should also reflect everyday needs for a specific item.
\end{tcolorbox}

% 简单色块
\begin{tcolorbox}[colback=green!10, colframe=green!80!black, title=common sense]
\textbf{\{Here, different tasks have different descriptions and emphases. For details, please refer to the code.\}}\\
Please find the target entity's specific character which is different with other target objects and combine into the instruction.\\
\textbf{\{Here are the examples for each task.\}}\\
Please provide the task following the format of the above example.
Please provide ten tasks that meet the above requirements and format.
\end{tcolorbox}


\begin{tcolorbox}[colback=green!10, colframe=green!80!black, title=Semantic]
Please find target entity's specific character which is different with other target objects and combine into the instruction.
Do not directly mention the target entity by name and avoid explicitly stating the need for the object. Instead, create tasks that reflect real-life scenarios where the need for the object is implied through casual, everyday observations. The task should suggest a need without saying it directly, focusing on natural, implied requests.  
\textbf{\{Here are the examples for each task.\}}\\
Please provide the task following the format of the above example.\\
The target\_entity must be the target entity. Please provide ten tasks that meet the above requirements and format.
\end{tcolorbox}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%complex task
\begin{tcolorbox}[colback=green!10, colframe=green!80!black, title=Dining Table Set]
The current task involves a dining scenario where the robot arm needs to set the dining table. Please design real-life scenarios that require setting a dining table, and generate corresponding instructions based on the specific table setting requirements.\\
You cannot specify the exact how to set table; just create a realistic scenario that requires to set dining table.\\
Please make the generated instructions more diverse in terms of conversational language, tone, and scenarios. Avoid sticking to a single sentence structure.\\
\textbf{\{Here are the examples for each task.\}}\\
Please provide the task following the format of the above example.\\
Please provide ten tasks that meet the above requirements and format.
\end{tcolorbox}

\begin{tcolorbox}[colback=green!10, colframe=green!80!black, title=Get Black Coffee]
Now, you need to design tasks that require black coffee. Please create real-life scenarios where there is a need for black coffee and generate corresponding instructions based on the specific need for black coffee.\\
Please make the generated instructions more diverse in terms of conversational language, tone, and scenarios. Avoid sticking to a single sentence structure.\\
\textbf{\{Here are the examples for each task.\}}\\
Please provide the task following the format of the above example.\\
Please provide ten tasks that meet the above requirements and format.
\end{tcolorbox}

\begin{tcolorbox}[colback=green!10, colframe=green!80!black, title=Get Coffee With Sugar]
Now you need to create a task that requires a coffee with sugar. Please design real-life scenarios where there is a need for coffee with added sugar, and generate an instruction based on the combined need for both sugar and coffee. \\
Be sure to incorporate the need for sugar along with the coffee in the instruction.\\
Please make the generated instructions more diverse in terms of conversational language, tone, and scenarios. Avoid sticking to a single sentence structure.\\
\textbf{\{Here are the examples for each task.\}}\\
Please provide the task following the format of the above example.\\
Please provide ten tasks that meet the above requirements and format.
\end{tcolorbox}

\begin{tcolorbox}[colback=green!10, colframe=green!80!black, title=Cluster Book]
The task now is to classify the books. Please design real-life scenarios where there is a need to categorize books, and generate an instruction based on the classification requirement. \\
You cannot specify the exact classification method; just create a realistic scenario that requires classification and instruct it to categorize the books in front of it.\\
Please make the generated instructions more diverse in terms of conversational language, tone, and scenarios. Avoid sticking to a single sentence structure.\\
\textbf{\{Here are the examples for each task.\}}\\
Please provide the task following the format of the above example.\\
Please provide ten tasks that meet the above requirements and format.
\end{tcolorbox}

\begin{tcolorbox}[colback=green!10, colframe=green!80!black, title=Texas Holdem Play]
There is currently a scenario where Texas Hold'em poker is being played, and you need to design a task for the robotic arm to select the highest-ranking hand. Please create a realistic poker-playing scenario and clearly instruct it to choose the best possible hand to play, generating the corresponding instruction.\\
Please make the generated instructions more diverse in terms of conversational language, tone, and scenarios. Avoid sticking to a single sentence structure.\\
\textbf{\{Here are the examples for each task.\}}\\
Please provide the task following the format of the above example.\\
Please provide ten tasks that meet the above requirements and format.
\end{tcolorbox}


\begin{tcolorbox}[colback=green!10, colframe=green!80!black, title=Rearrange Book By Year]
The task now is to organize the books by publication year. Please design real-life scenarios where there's a need to arrange books by year, and create instructions based on the sorting requirement.\\
Please make the generated instructions more diverse in terms of conversational language, tone, and scenarios. Avoid sticking to a single sentence structure.\\
\textbf{\{Here are the examples for each task.\}}\\
Please provide the task following the format of the above example.\\
Please provide ten tasks that meet the above requirements and format.
\end{tcolorbox}

\begin{tcolorbox}[colback=green!10, colframe=green!80!black, title=Cook Dishes]
Please change the dish names in the sentences above to descriptions that better fit a real-life context and integrate these descriptions into instructions that convey the need for that particular dish.\\
\textbf{\{Here are the examples for each task.\}}\\
Please provide the task following the format of the above example.\\
Please provide ten tasks that meet the above requirements and format.
\end{tcolorbox}

\begin{tcolorbox}[colback=green!10, colframe=green!80!black, title=Heat Food]
The task now is to heat the food on the tray. Please design real-life scenarios where food on a tray needs to be heated, and clearly instruct to heat the food. \\
Avoid mentioning what specific food to heat.\\
Please make the generated instructions more diverse in terms of conversational language, tone, and scenarios. Avoid sticking to a single sentence structure.\\
\textbf{\{Here are the examples for each task.\}}\\
Please provide the task following the format of the above example.\\
Please provide ten tasks that meet the above requirements and format.
\end{tcolorbox}

\begin{tcolorbox}[colback=green!10, colframe=green!80!black, title=Get Cool Drink]
Please create real-life scenarios where there is a desire for a cold drink, and based on the need for these drinks, generate the corresponding instructions.\\
Please emphasize that the drink should be cold.\\
Please make the generated instructions more diverse in terms of conversational language, tone, and scenarios. Avoid sticking to a single sentence structure.\\
\textbf{\{Here are the examples for each task.\}}\\
Please provide the task following the format of the above example.\\
Please provide ten tasks that meet the above requirements and format.
\end{tcolorbox}

\begin{tcolorbox}[colback=green!10, colframe=green!80!black, title=Study Table Set]
Please design real-life scenarios where you need to use the above-mentioned target entities for learning and clearly instruct to tidy up the desk and turn on the computer.\\
Please make the generated instructions more diverse in terms of conversational language, tone, and scenarios. Avoid sticking to a single sentence structure.\\
\textbf{\{Here are the examples for each task.\}}\\
Please provide the task following the format of the above example.\\
Please provide ten tasks that meet the above requirements and format.
\end{tcolorbox}

\begin{tcolorbox}[colback=green!10, colframe=green!80!black, title=Take Chemistry Experiments]
Now, please generate tasks for the robotic arm based on the following requirements.\\
First, extract the chemical reaction solutions from within the sentence :xxx. \\
And create instructions with a chemical experiment context, specifying the need for the given reaction solutions.\\
Please incorporate the requirement to find these reaction solutions into the instruction.\\
Please include the requirement for all reaction solutions in the instruction. Generate 5 tasks for this part.\\
Secondly, extract the chemical properties of the products within the sentence from the chemical reactions, such as precipitate, gas, color, etc. In this case, do not specify the reaction solutions; instead, only reference the products to create the instructions. These should also be framed in the context of a chemical experiment. \\
Please incorporate the requirement to find the reaction solution into the instruction.\\
Please emphasize in the instruction that the final reaction should yield the specified products. Generate 5 tasks for this part.\\
\textbf{\{Here are the examples for each task.\}}\\
Please provide the task following the format of the above example.
\end{tcolorbox}

==> table/table_for_poster.tex <==
\begin{table}[h!]
    % \centering  
    \begin{subtable}[t]{0.24\textwidth}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cccc}
        % First large table content remains the same
        \hline
       \textbf{Model} & \textbf{Task Name} & \textbf{Seen} & \textbf{Unseen} \\ \hline
        \multirow{2}{*}{Octo} & Base & 1.34 & 0.77 \\ 
        & Common Sense & 1.16 & 0.96\\
        \hline
        \multirow{2}{*}{OpenVLA} & Base & 11.74 & 7.93\\ 
        & Common Sense & 8.46 & 5.11\\ \hline
        \multirow{2}{*}{RDT-1B} & Base & 15.37 & 9.08\\ 
        & Common Sense & 11.97 & 3.61\\ \hline
    \end{tabular}}
    \caption{Evaluation of visual generalization and knowledge transfer.}
    \label{subtable:exp1}
    \end{subtable}
    \vfill
    \begin{subtable}[t]{0.24\textwidth}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{p{3cm}ccc}
        \hline
        \textbf{Task} & Octo & OpenVLA & RDT-1B\\ \hline
        Add Condiment & 0.00 & 0.00 & 6.15 \\
        Insert Flower & 0.00 & 10.00 & 9.24 \\
        Select Drink & 0.00 & 7.69 & 3.08 \\
        Select Toy & 0.00 & 0.00 & 3.08 \\
        Select Tube & 0.00 & 3.08 & 0.00 \\
        Average& \textbf{0.00} & \textbf{4.15} & \textbf{4.31} \\
        \hline 
    \end{tabular}
    }
    \caption{Evaluation of language instruction generalization.}
    \label{subtable:exp2}
    \end{subtable}

    
    \begin{subtable}[t]{0.24\textwidth}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{p{3cm}ccc}
        \hline
        \textbf{Task} & Octo & OpenVLA & RDT-1B\\ \hline
        Select Poker & 0.00 & 7.69 & 4.62 \\
        Select Majhong & 0.00 & 4.62 & 3.07 \\
        Select Billiards & 0.00 & 3.07 & 4.62 \\
        Select Ingredient & 0.00 & 0.00 & 0.00 \\
        Friction QA & 0.00 & 10.46 & 6.92 \\
        Average& \textbf{0.00} & \textbf{4.46} & \textbf{3.85} \\
        \hline 
    \end{tabular}
    }
    \caption{Evaluation of unseen but similar task generalization.}
    \label{subtable:exp3}
    \end{subtable}
    \vfill
    \begin{subtable}[t]{0.24\textwidth}
    % \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{p{3cm}ccc}
        \hline
        \textbf{Task} & Octo & OpenVLA & RDT-1B\\ \hline
        Find Unseen Object & 0.00 & 7.69 & 0.00 \\
        Play Texas Holdem & 0.00 & 3.54 & 3.08 \\
        Cluster Toy & 0.00 & 0.00 & 5.06 \\
        Hammer and Hang & 0.00 & 0.00 & 0.00 \\
        Get Latte Coffee & 0.00 & 2.08 & 8.56 \\
        Average& \textbf{0.00} & \textbf{2.66} & \textbf{3.34} \\
        \hline 
    \end{tabular}
    }
    \caption{Evaluation of composite tasks.\newline}
    \label{subtable:exp4}
    \end{subtable}

    \caption{Overall experiment result of generalization ability of fine-tuned VLAs.}
    \label{table:vla-exp}
\end{table}
% \vspace{}
